Achieving Realistic Cyclist Behavior in SUMO using the SimRa Dataset

Increasing the modal share of bicycle traffic to reduce carbon emissions, reduce urban car traffic, and to improve the health of citizens, requires a shift away from car-centric city planning. For this, traffic planners often rely on simulation tools such as SUMO which allow them to study the effects of construction changes before implementing them. Similarly, studies of vulnerable road users, here cyclists, also use such models to assess the performance of communication-based road traffic safety systems. The cyclist model in SUMO, however, is very imprecise as SUMO cyclists behave either like slow cars or fast pedestrians, thus, casting doubt on simulation results for bicycle traffic. In this paper, we analyze acceleration, deceleration, velocity, and intersection left-turn behavior of cyclists in a large dataset of real world cycle tracks. We use the results to improve the existing cyclist model in SUMO and add three more detailed cyclist models and implement them in SUMO.

==> content/acronyms.tex <==
\acrodef{5G}{Fifth Generation}
\acrodef{ANN}{Artificial Neural Network}
\acrodef{AUC}{Area under the curve}
\acrodef{BCE}{Binary Crossentropy}
\acrodef{CNN}{Convolutional Neural Network}
\acrodef{DFT}{Discrete Fourier Transform}
\acrodef{FPR}{False Positive Rate}
\acrodef{GDPR}{General Data Protection Regulation}
\acrodef{GRU}{Gated Recurrent Unit}
\acrodef{HAR}{Human Activity Recognition}
\acrodef{IQR}{Interquartile Range}
\acrodef{LSTM}{Long Short-Term Memory}
\acrodef{OSM}{Open Street Map}
\acrodef{OS}{Operating System}
\acrodef{RELU}{Rectified Linear Unit}
\acrodef{RNN}{Recurrent Neural Network}
\acrodef{ROC}{Receiver operating characteristic}
\acrodef{SAS}{Sensitivity at Specificity}
\acrodef{SF}{Sensor-based Fusion}
\acrodef{SGD}{Stochastic Gradient Descent}
\acrodef{TPR}{True Positive Rate}

